MultiTEND: A Multilingual Benchmark for Natural Language to NoSQL Query Translation

Natural language interfaces for NoSQL databases are increasingly vital in the big data era, enabling users to interact with complex, unstructured data without deep technical expertise. However, most recent advancements focus on English, leaving a gap for multilingual support. This paper introduces MultiTEND, the first and largest multilingual benchmark for natural language to NoSQL query generation, covering six languages: English, German, French, Russian, Japanese and Mandarin Chinese. Using MultiTEND, we analyze challenges in translating natural language to NoSQL queries across diverse linguistic structures, including lexical and syntactic differences. Experiments show that performance accuracy in both English and non-English settings remains relatively low, with a 4%-6% gap across scenarios like fine-tuned SLM, zero-shot LLM, and RAG for LLM. To address the aforementioned challenges, we introduce MultiLink, a novel framework that bridges the multilingual input to NoSQL query generation gap through a Parallel Linking Process. It breaks down the task into multiple steps, integrating parallel multilingual processing, Chain-of-Thought (CoT) reasoning, and Retrieval-Augmented Generation (RAG) to tackle lexical and structural challenges inherent in multilingual NoSQL generation. MultiLink shows enhancements in all metrics for every language against the top baseline, boosting execution accuracy by about 15% for English and averaging a 10% improvement for non-English languages.

==> Table/Ablation_Study.tex <==

\begin{table*}[htbp!]
    \captionsetup{width=\textwidth}
    \centering
    \scalebox{1.0}{
    \begin{tabular}{l|ccc|ccc}
    \toprule
    & \multicolumn{3}{|c|}{\textbf{Query-based}} & \multicolumn{3}{c}{\textbf{Execution-based}} \\
    \midrule
    \textbf{Method} & EM & QSM & QFC & EX & EFM & EVM \\
    \midrule
    Few-Shot LLM & 5.91\% & 50.77\% & 64.32\% & 35.06\% &  53.05\%  & 58.23\% \\
    RAG for LLM & 37.74\% & 62.10\% & 51.57\% & 57.02\% &  74.61\%  & 71.29\% \\
    \textbf{UniLink (Ours)} & 23.82\% & 63.21\% & 75.60\% & \textbf{65.08\%} &  \textbf{87.21\%}  & \textbf{72.79\%} \\
    $\quad$ - w/o Sk-G & 23.78\% & 63.53\% & \textbf{76.65\%} & 63.78\% &  85.80\%  & 71.24\% \\
    $\quad$ - w/o SL-G & \textbf{24.07\%} & \textbf{63.64\%} & 75.28\% & 62.85\% &  87.17\%  & 70.88\% \\
    $\quad$ - w/o AUG  & 23.06\% & 63.21\% & 75.71\% & 63.78\% &  86.85\%  & 72.47\% \\
    $\quad$ - only GEN & 20.54\% & 56.50\% & 67.68\% & 53.12\% &  84.36\%  & 68.11\% \\
    
    \bottomrule
    \end{tabular}}
    \caption{Ablation study results on the MultiTEND test set. This table shows the performance of UniLink on various metrics after removing each component.}
    \label{tab:ablation_study}
    \vspace{-25pt}
\end{table*}

==> Table/Dataset_Statistics.tex <==
\begin{table*}[!h]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \begin{adjustbox}{max width=\textwidth} % 调整表格宽度以适应页面
        \begin{tabular}{>{\raggedright\arraybackslash}m{5.5cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{3cm}}
            \toprule
            Dataset & Task & NLQ & Query & Domain & Languages  \\
            \midrule
            Spider~\cite{min2019pilot} & Text-to-SQL & 10,181& 5,693 & 138 & English \\
            nvBench~\cite{luo2021synthesizing} & Text-to-Vis & 25,750 & 7,247 & 105 & English \\
            OverpassQL~\cite{staniek2023text} & OpenStreeMap Querying & 8,352 & 3,890 & - & English \\
            {Tend} & Text-to-NoSQL & 16,540 & 3,308 & 105 & English  \\
            \textbf{MultiTend} & Multilingual Text-to-NoSQL & \textbf{99,240} & \textbf
{19,848} & 105 & \textbf{Multiple (6)} \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Comparison between existing datasets and MultiTend benchmark}
    \label{table:comparison_datasets}
    \vspace{-15pt}
\end{table*}
